MC-GAN: Multi-conditional Generative Adversarial Network for Image Synthesis

In this paper, we introduce a new method for generating an object image from text attributes on a desired location, when the base image is given. One step further to the existing studies on text-to-image generation mainly focusing on the object's appearance, the proposed method aims to generate an object image preserving the given background information, which is the first attempt in this field. To tackle the problem, we propose a multi-conditional GAN (MC-GAN) which controls both the object and background information jointly. As a core component of MC-GAN, we propose a synthesis block which disentangles the object and background information in the training stage. This block enables MC-GAN to generate a realistic object image with the desired background by controlling the amount of the background information from the given base image using the foreground information from the text attributes. From the experiments with Caltech-200 bird and Oxford-102 flower datasets, we show that our model is able to generate photo-realistic images with a resolution of 128 x 128. The source code of MC-GAN is released.

==> 1_Introduction.tex <==
\section{Introduction}
\label{sec:intro}
사람이 한가지 종류의 정보만 이용하지 않고 여러종류를 이용하는 것 처럼 딥러닝 연구도 다양한 종류의 데이터를 이용하는 연구가 활발하다 \cite{VQA,santoro2017simple,chang2017broadcasting}. Classification research area 뿐만 아니라 Generative model realm 에서도 다른 종류의 데이터를 조건으로 주어 이미지를 만드는 연구가 Generative Adversarial Network (GAN) 이용하여 진행되고 있다. 예를 들어object 를 설명하는 text 이용하거나 object의 위치를 지정하여 이미지를 생성하기도 하며, 원래의 이미지를 다른 domain style 로 transfer 하거나 \cite{DBLP:conf/nips/MaJSSTG17,choi2017stargan} label map 을 실제 이미지로 바꿔주는 연구들이 있다 \cite{wang2018pix2pixHD}.

% 사람은 한가지 종류의 정보만 인식하지 않고 여러 종류의 정보를 함께 고려하여 인지를 하게 된다. 사람의 뇌를 모방한 딥러닝 연구도 uni-modal problem 에서 벗어나 Visual QnA, Relation Network \cite{VQA,santoro2017simple,chang2017broadcasting} 등 multi-modal problem을 다루기 시작했다.
% \yj{위의 연구들이 인간의 인지를 모방한 것인지? 그냥 여러 data를 활용하려 한거 아닌가요?}
% \hj{사람처럼 다양한 정보를 이용할려는 거니까 인지를 모방?? }
% 또한 사람은 주어진 정보를 인식하는 것이 아니라 상상하여 새로운 정보도 만들 수 있다. 이를 모방한 다른 딥러닝 연구로는 Generative model 이 있다. 최근 Generative model 은 Generative Adversarial Network (GAN) 을 이용하여 단순히 random 한 큰 이미지를 만드는 것이 아니라 주어진 condition 을 이용해서 이미지를 만드는 연구도 활발히 진행되고 있다.
% \yj{보통 Image generation 모델 인트로 할 때는 모방 보다는 image의 특성을 modeling하고, 이를 통해 새로운 이미지를 생성할 수 있는... 이런 느낌으로 목적이 나옴.}
% \hj{multi-modal condition 쪽을 강조하고 싶어서 이렇게 인트로를 했는데 어떻게 하는게 좋을까요?}

그러나 앞서 언급한 conditional GAN 연구에서 1) multi-modal condition을 주어 이미지를 생성하는 연구는 조건들이 뒤섞여 이상한 이미지를 만들어내는 경우가 많아 한가지 종류의 조건을 사용한 것 보다 기술적으로 어렵다. 또한 넣어주는 조건들이 2) object 에 대한 것이고 background 에 대한 control 은 불가능하다. 즉 사용자들이 원하는 base에 추가적인 object 만 합성하여 쓰고 싶은 경우가 많지만 이에 대한 연구는 거의 없다. 최근에 multi-modal condtition GAN 연구가 몇가지 진행되었으나 위 문제들을 종합적으로 해결해주지 못한다.  \cite{reed2016learning} 은 Text 와 원하는 object 의 위치를 지정해주면 이미지를 생성해주지만 배경에 대한 control을 할 수 없다. \cite{dong2017semantic} 는 Text와 이미지 조건을 함께 고려하여 object과 관련 없는 부분을 control 할 수 있지만, 만들려는 object가 이미 Base image 에 있어야 하는 제약조건이 있으며, base-object가 input text condition 에 따른 style transfer 문제이다.



% \hj{교수님: base 에 대한 제대로 정의가 필요 간단한 그림을 추가하자 비교논문 그림까지}
% 그러나 대부분 연구는 1) 이미지 혹은 Text 한가지 종류의 condition 만 가능하며, 2) 또한 이미 사용자가 가지고 있는 Base에 추가적인 정보를 더하여 합성하는 연구는 거의 없다. 
% \yj{무슨 이유로 없는지? 위 내용이 만족되면 아래 내용은 간단히 정리만 하고 related work으로 넘길 수 있음.}
% \hj{어려워서 --? 잘 말을 못하겠습니다.}
% 최근에 multi-modal condition 연구가 시작되었으나  불편한 제약 조건이 있다. \cite{reed2016learning} 은 Text 와 원하는 object 의 위치를 지정해주면 이미지를 생성해주지만 사용자가 가지고 있는 \hj{교수님:Base가 무엇인지에 대해 잘 알수가 없음 Base} 를 반영하는 연구가 아니다. \cite{dong2017semantic} 는 Text와 이미지 조건을 함께 고려하는 더 어려운 문제를 풀지만, \hj{교수님: style 변경문제라고 말하는 것이 좋음} 만들려는 object가 이미 \ Base image 에 있어야 하며 이 base-object가 input text condition 에 따라 전환하는 단순한 문제이다. 결론적으로 기존의 연구들 중 사용자가 object 가 없는 base-image 줄 때, multi-modal condition을 이용하여 이미지를 합성하는 종합적인 목표를 가진 것은 없다.  
% \yj{그렇다면 이 연구는 어떠한 의미가 있는가?}
% \hj{다음단락에 종합적으로 해결한다고 하니까 ㅇㅇ???}
% \yj{이러한 연구의 practical 의미와 기술적으로 넘어야 할 과제}
% \hj{배경과 새로생긴 obj가 섞이지 않아야 하고 obj 도 이쁘게 잘 나와야 한다???}
% \yj{To tackle the mentioned problems,}

To tackle the mentioned problems, 본 연구의 main contribution 은 위에 언급한 두가지 문제를 종합적으로 해결하는 새로운 multi-modal condition synthesis 문제를 지적하며 이를 효과적으로 다루는 Synthesis-block 을 제안한다. 우리가 정의하는 문제는 Base image 에 object가 있을 필요 없이 원하는 배경 이미지와 위치 그리고 원하는 object를 설명하는 text로 이미지 생성을 가능하게 한다. 원하는 배경 이미지와 생성하고 싶은 위치를 정해주면, 배경을 반영하여 적절한 pose를 가진 object 를 text 내용에 맞게 생성을 한다. 또한 배경을 단순히 복사하는 것이 아니라 필요에 따라 생성되는 object에 맞추어 배경을 자연스럽게 변경한다. 이를 통해 우리는 복잡한 multi-modal condition GAN 문제와 object, background 를 동시에 control 할 수 있는 의미를 지닌다.

위에서 정의한 새로운 합성 문제를 해결하기 위해 우리는 Residual block 에서 아이디어를 가져온 Synthesis Block 을 사용한 generator network 와 discriminator network를 제안한다.  또한  이 Synthesis block 이 input base-image 에서 object 여부와 관계없이 image-text condition 문제에 모두 쓰일 수 있음을 보인다. 우리는 Caltech-200 bird dataset \cite{WahCUB_200_2011} 과 Oxford-102 flower dataset \cite{Nilsback08} 을 이용하여 기존의 비슷한 문제를 언급한 \cite{dong2017semantic} 을 baseline method 로 함께 비교한다. 


% 대표적인 conditional Gan 연구는 text를 이용하여 이미지를 만들거나, 기존의 이미지의 domain 을 바꾸는 것들 것 있다. 그러나 condition이 하나의 종류에만 제한되어 있으며, multi-modal condition 연구는 부족하다. 또한 Gan 결과를 실제에 적용하기 위해서는 모든 이미지를 만들어주기 보다는 사용자가 원하는 곳에 기존의 정보를 반영하여 합성하는 것이 가능해야 한다. 최근 이런 문제를 고려한 multi-modal 연구가 시작되었다. \cite{dong2017semantic} 는 만들려는 object가 있는 base image에서, 새로운 FG를 설명하는 text 를 넣어주면 base image의 object의 pose와 배경의 분위기가 유지되면서 text에 기반한 새로운 이미지가 생성된다. 그러나 이 연구는 입력 이미지에 object가 있어야 하는 제약사항이 있다. 하지만 우리 연구는 원하는 배경 이미지와 생성하고 싶은 위치를 정해주면, 배경을 반영하여 적절한 pose를 가진 object 를 생성을 하고 필요에 따라 생성되는  object에 맞추어 배경을 변경해준다. 
% \yj{기존의 알고리즘의 문제점은 무었이고 본 알고리즘에서는 어떠한 문제를 tackle 하고 싶은것인지?}
% \yj{이 문제를 해결하기 위해 Here, 우리는 A, B, C를 제안하고 걔네들에 대한 설명과 효과.}



==> 2_RelatedWork.tex <==
\section{Related Work}
\label{related_work}
%최근 GAN 연구는 random noise 에서 random 한 이미지를 만드는 문제에서 벗어나 주어진 condition 에 따라 생성할 이미지를 control 할 수 있도록 발전하였다. 이러한 Conditional GAN 연구는 크게 다음과 같이 나눌 수 있다. 1) style transfer problem 2) text to image problem 3) multi-modal condition problem.

Style transfer problem 은 input으로 보통 이미지를 이용하며 전경을 다른 스타일로 바꿔주는 work 이다. 예를 들어 웃는 얼굴을 화난 얼굴로 바꾸거나, 핸드백을 신발로 바꾸는 등 다른 domain 의 스타일로 바꾸는 것이 대표적이다 \cite{CycleGAN2017, choi2017stargan, kim2017disco}. 이 뿐만 아니라 segmentation label map 에 맞게 real image 만드거나 \cite{wang2018pix2pixHD, chen2017photographic}, part location map 과 원래의 사람 이미지를 input 으로 이용하여 다른 pose를 가진 사람으로 만들어주는 것도 style transfer problem 으로 볼 수 있다. 
Text to image problem 은 input 으로 object 를 설명해주는 text 를 input 으로 이용하여 text 내용에 맞게 이미지를 생성한다. 보통 text embedding 방식으로는 hybrid CNN-RNN structure 를 이용한  \cite{reed2016txt_emb} 를 따른다. \cite{reed2016generative} 이 처음으로 이를 제안하였으며 후에 이미지 quality 를 향상시킨 \cite{zhang2017stackgan, Han17stackgan2} work들이 있다.

\noindent
\textbf{Conditional Image Generation: }
Multi-modal condition problem 은 image-location or image-text 등 다른 종류의 input condition에 맞게 이미지를 생성하는 것을 말한다. \cite{reed2016learning}은 단순히 text 조건에서 이미지를 생성하는 것이 아니라 생성 될 이미지에서 원하는 object의 위치를 bounding box 를 통해 지정하거나 원하는 part location 을 point로 지정하여 text와 위치조건 2가지를 함께 고려하여 이미지를 생성한다. \cite{dong2017semantic} 은 이미지와 텍스트 두 종류의 정보를 조건으로 가진다. \cite{dong2017semantic}는 input base image 에 object가 이미 있어야 하며, text 와 관련없는 부분은 유지하고 text와 관련있는 object의 모습을 text 에 맞게 style을 바꾸는 것이 목적이다. 

\cite{reed2016learning} 는 위치 정보를 이용한다는 점에서 비슷하나, 우리의 연구는 넣어준 배경 이미지의 semantic 정보를 이해하여 object 를 생성하기 때문에 사용자가 임의로 part location을 선택하여 pose 까지 지정해주는 것은 부자연스러울 수 있다. 그러나 bounding box를 조건을 주는 것은 배경이미지에서 위치를 지정해주는 것과 비슷하므로, 우리의 연구는 부분적으로 \cite{reed2016learning} 에서 정의한 문제까지 포함한다. \cite{dong2017semantic} 는 image-text 조건을 함께 쓴다는 점에서 비슷하나 우리의 연구는 base image 에 object 가 있어야 하는 조건에서 자유롭다. 즉 style 변경이 아니라 배경을 유지하면서 text 정보에 따라 생긴 새로운 object 를 만들기 때문에 서로 정의한 문제가 다르며 우리의 연구가 합성이란 관점에서 좀 더 알맞다.

언급한 알고리즘들과 달리, 제안하는 알고리즘은 다음과 같은 효과를 가진다. 1) input 으로 base image, location, text를 가지며 배경을 유지하면서 text의 attribute에 맞게 object 이미지를 원하는 위치에 생성한다. 2) 이때 object는 배경에 맞는 알맞은 pose를 가지고 생성되며, 또한 단순히 배경을 copy 하는 것이 아니라 필요한 경우 적절한 변화를 준다. 3) 이를 통해 base image에 object가 없는 경우에도 원하는 object를 base image에 자연스럽게 추가할 수 있으며 전경과 배경을 두가지를 모두 control 할 수 있다는 장점이 있다. 실제환경에서 base image에 우리가 원하는 object가 존재하는 경우가 많이 없고, 기존의 image transfer 알고리즘들이 배경을 적절히 유지하면서 object의 shape만 효과적으로 바꾸지는 못한다는 점에서 어려운 문제이다.



% \yj{좀 더 간단하게 한문장을 가능}
% computer vision은 단순히 vision 만 이용하는 것 아니라 어떤 문장을 넣어주면 문장을 이해하여 의미하는 것을 이미지에 찾는 문제나 이미지에 있는 물체들의 Relation 을 고려하여 문장에 답을 해주는 종합적인 문제에 접근하기 시작했다 \cite{VQA, santoro2017simple, chang2017broadcasting}. 또한 classification 문제에서 벗어나 새로운 데이터를 만드는 연구도 활발해졌는데 가장 대표적인 방법론으로는 GAN  이 있다.

% GAN 은 학습이 불안정하여 mode collapse 문제가 일어나는데 이를 해결하여 이미지의 quality 를 향상시키는 연구가 추후에 많이 진행되었다\yj{우리 문제가 mode collapse를 푸는 것이 아니라면 굳이 언급할 필요 없음}. ~\cite{mao2017least, radford2016unsupervised,Han17stackgan2}. 
% 또한 random 하게 생성하는 것이 아니라 원하는 condition 의 object를 생성해주는 연구도 함께 진행 되었다 \cite{chen2016infogan, wang2018pix2pixHD, reed2016generative,DBLP:conf/nips/MaJSSTG17}. 
% \yj{아래 주어가 없는 문장들이 있는데 check. 논문들이 단순히 나열되고 있는 느낌이 들기 때문에 제안하는 연구와 관련된 것과 그렇지 않은 일반적인 내용 (간단하게) 으로 문단을 나누어 확실히 비교할 필요가 있음}
% 특히 원하는 object의 모습을 text 로 설명한 문장을 noise 와 섞어 다양한 이미지를 만드는 시도로 \cite{reed2016generative}가 시작하였다. 
% 이를 발전시킨 \cite{reed2016learning}은 단순히 text 조건에서 이미지를 생성하는 것이 아니라 생성 될 이미지에서 원하는 object의 위치를 bounding box 를 통해 지정하거나 원하는 part location 을 point로 지정하여 text와 위치조건 2가지를 함께 고려하여 이미지를 생성한다. 
% 위치 정보를 이용한다는 점에서 비슷하나, 우리의 연구는 넣어준 배경 이미지의 semantic 정보를 이해하여 object 를 생성하기 때문에 사용자가 임의로 part location을 선택하여 pose 까지 지정해주는 것은 부자연스러울 수 있다. 
% 그러므로 bounding box를 조건을 주는 것은 배경이미지에서 위치를 지정해주는 것과 비슷하므로, 우리의 연구는 부분적으로 \cite{reed2016learning} 에서 정의한 문제까지 포함한다.

% \yj{\cite{dong2017semantic}, \cite{reed2016generative} 이런 유사한 논문들의 주제를 한 category로 설명한다면? 문단 나누고 \textbf{분류:} 이런 식으로 해당 문단에 대한 강조를 해주어도 좋음.}
% \hj{ text 를 이용한 GAN (text2 img GAN, stack GAN 에 대해 설명), multi-modal GAN 이렇게(what2where, iccv) 두개로???}
% \cite{dong2017semantic} 은 \cite{reed2016generative} 를 기반으로 한 모델로, 이미지와 텍스트 두 종류의 정보를 조건으로 가진다는 점에서 우리의 연구와 비슷하다. 두 연구 모두 object 와 관련 없는 이미지 부분은 유지한다는 점에서는 비슷하나 \cite{dong2017semantic}는 input base-image 에 object가 이미 있어야 하는 조건이 있고, 이 object의 모습을 text 에 맞게 바꾸는 것이 목적이다. 
% 우리의 연구는 object가 있을 필요 없이 배경 이미지만 넣어주면 되며, 배경을 유지하지만 새로 생긴 object 에 따라 조금씩 변한다. 또한 텍스트 정보에 따라 생긴 새로운 object도 배경에 맞는 위치와 pose를 가지고 서로 합성하는 것을 목적으로 가지기 때문에 서로 정의한 문제가 다르다. 특히 base-image 를 이용한 이미지 합성이라는 관점에서는 이전 연구의 조건인 base-image에 object가 있어야하는 제약 조건에서 자유로워졌으며 우리가 제안한 synthesis block 은 \cite{dong2017semantic}가 정의한 문제에서도 충분히 쓰일 수 있음을 실험적으로 증명한다.
% \yj{우리의 연구 이하 내용을 ....}
% \yj{언급한 알고리즘들과 달리, 제안하는 알고리즘은 base image에 오브젝트가 있는 경우 뿐 만아니라 배경만 있는 경우에도 text로 주어지는 attribute에 맞게 object 이미지를 the base image의 원하는 위치에 생성하는 것을 목표로 하고 있다. (문장 나누어서)
% 이를 통해 base image에 object가 없는 경우에도 원하는 object를 base image에 자연스럽게 추가할 수 있는 장점이 있다. 
% 이는 실제 base image에 우리가 원하는 object가 존재하는 경우가 많이 없고, 기존의 image transfer (cycle gan 등...)의 알고리즘들이 object의 shape를 효과적으로 바꾸지는 못한다는 점에서 어려운 문제이다.
% --이런 느낌으로 작성해도 좋을듯
% }


%\yj{우리 알고리즘과 다른 점은?}

==> 3_Background.tex <==
\section{Background}
\label{sec:Background}

\subsection{Generative Adversarial Networks}
\label{sec:GAN}
Generative Adversarial Network (GAN)\cite{goodfellow2014generative} 은 fake image 를 만드는 generator 와 이를 감별해내는 discriminator 로 구성된다.  Generator 는 true data distribution $P_{data}$ 를 학습하여 random seed로 진짜 같은 이미지를 생성한다.반면에 discriminator 는 이를 구별해낼려고 하기 때문에 결국 두 네트워크는 two-player min-max game 으로 볼 수 있으며 Eq \ref{eq:gan}. 으로 formulated 된다.
\begin{equation}
\small
\min_{G} \max_{D} V(D,G) \; = \; \mathds{E}_{x\sim p_{data}(x)}\;[\, \log{D(x)} \, ] \; + \; \mathds{E}_{z\sim p_{z}(z)}\;[\, \log{1 - D(G(z))}\, ]
\label{eq:gan}
\end{equation}

그러나 두 네트워크가 싸우는 특징 때문에 GAN 은 학습이 불안정하다는 문제가 있다. 특히 discriminator의 sigmoid 함수로 인해 gradient vanishing problem 이 발생한다. 이를 해결하기 위해 Mao \etal \cite{mao2017least} 는 least squares loss function 을 discriminator 에 적용하였으며, 이 방법이 $Pearson \; \chi ^{2}$ 를 minimization 하는 것과 같다는 것을 증명하였다. 결론적으로 Eq \ref{eq:gan}. 은 Eq \ref{eq:LSgan}. 으로 변경하여 굉장히 쉬운 방법으로 안정적인 학습이 가능해졌다.


\begin{equation}
\small
\begin{gathered}
\min_{D} V(D) \; = \; 0.5\; \mathds{E}_{x\sim p_{data}(x)}\;[\, ({D(x)-1})^2 \,]
\; + \; 0.5\; \mathds{E}_{z\sim p_{z}(z)}\;[\, {D(G(z))}^2 \, ] \\
\min_{G} V(G) \; = \; 0.5\; \mathds{E}_{z\sim p_{z}(z)}\;[({D(G(z))-1})^2]
\label{eq:LSgan}
\end{gathered}
\end{equation}


\subsection{Text Embedding}
\label{sec:txt}

\cite{reed2016txt_emb} designed a hybrid CNN-RNN model to retrieve desired images through texts.
\cite{reed2016generative,reed2016learning} make more improved model to generate image from text description.
Since text embedding is a high dimension but the number of data is small, \cite{zhang2017stackgan,Han17stackgan2} points out that latent space has a discontinuity problem.
For this reason, they use text embedding $\varphi_{t}$ to find independent conditioning Gaussian distribution as latent space and propose Conditioning Augmentation to extract augmented sample by  $\hat{c_0} \; = \;  \mu_0 \, + \, \sigma_0 \odot \epsilon $ from new latent space. 
This allows us to solve the overfitting problem as well as to learn the conditioning manifold robustly from a small amount of image-text pair data by increasing various samples.
They apply Kullback-Leibler divergence (KL divergence) between the standard Gaussian distribution and the conditioning Gaussian distribution to the generator by Eq \ref{eq:txt}. for optimization. 
After $\hat{c_0}$ is concatenated with noise, the sample passes through a fully connected layer and becomes the desired spatial size for usage as a seed feature map.

\begin{equation}
\small
D_{KL} \; (\, N(\mu(\varphi_{t}), \; \Sigma(\varphi_{t} \,)\; || \; N(\,0, I\,))
\label{eq:txt}
\end{equation}


==> 3_Background_EN.tex <==
\section{Background}
\label{sec:Background}

\subsection{Generative Adversarial Networks}
\label{sec:GAN}
\yj{분량이 많은 경우 삭제 - every one knows this;; }
The Generative Adversarial Network (GAN) \cite{goodfellow2014generative} consists of a generator that creates fake images and a discriminator that separates real images from fake images. 
\yj{The} generator learns true data distribution $P_{data}$ to generate a real image from random seeds, whereas discriminator tries to distinguish it to \yj{the original images}. 
\yj{This framework} can be viewed as a two-player min-max game and are formulated as Eq \ref{eq:gan}.

\begin{equation}
\small
\min_{G} \max_{D} V(D,G) \; = \; \mathds{E}_{x\sim p_{data}(x)}\;[\, \log{D(x)} \, ] \; + \; \mathds{E}_{z\sim p_{z}(z)}\;[\, \log{1 - D(G(z))}\, ]
\label{eq:gan}
\end{equation}


However, training of GAN is unstable because the two networks are engaged in an ongoing \yj{conflict} to \yj{overwhelm} each other. 
%In particular, the discriminator’s sigmoid function causes a gradient vanishing problem. 
To alleviate the instability of the problem, a number of studies have been proposed. 
Mao \etal \cite{mao2017least} applied a least squares loss function to the discriminator and proved that this method is equivalent to minimizing $Pearson \; \chi^{2}$.
\yj{One more example such as w-gan.}

%In conclusion, Eq \ref{eq:gan}. is changed to Eq \ref{eq:LSgan}. and stable learning is possible in a very easy way.  \yj{It does not seems important I think?}

%\begin{equation}
%\small
%\begin{gathered}
%\min_{D} V(D) \; = \; 0.5\; \mathds{E}_{x\sim p_{data}(x)}\;[\, ({D(x)-1})^2 \,]
%\; + \; 0.5\; \mathds{E}_{z\sim p_{z}(z)}\;[\, {D(G(z))}^2 \, ] \\
%\min_{G} V(G) \; = \; 0.5\; \mathds{E}_{z\sim p_{z}(z)}\;[({D(G(z))-1})^2]
%\label{eq:LSgan}
%\end{gathered}
%\end{equation}




\subsection{Text Embedding}
\label{sec:txt}
\yj{이것도 분량 없음 날려도 될듯요}
Reed \etal \cite{reed2016txt_emb} designed a hybrid CNN-RNN model to retrieve desired images through sentences.
\cite{reed2016generative,reed2016learning} make more improved model to generate image from text description.
Since the vector \yj{generated} by the text embedding method \yj{lies on} high dimension \yj{manifold} and the number of data is small, \cite{zhang2017stackgan,Han17stackgan2} points out that \yj{There exsits a discontinuity in the mapped latent space.}
%latent space has a discontinuity problem.
For this reason, they use text embedding $\varphi_{t}$ to find\yj{find?} independent conditioning Gaussian distribution as latent space and propose Conditioning Augmentation to extract augmented sample by  $\hat{c_0} \; = \;  \mu_0 \, + \, \sigma_0 \odot \epsilon $ from new latent space. 
This allows us to solve the overfitting problem as well as to learn the conditioning manifold robustly from a small amount of image-text pair data by increasing various samples.
They apply Kullback-Leibler divergence (KL divergence) between the standard Gaussian distribution and the conditioning Gaussian distribution to the generator by Eq \ref{eq:txt}. for optimization. 
After $\hat{c_0}$ is concatenated with noise, the sample passes through a fully connected layer and becomes the desired spatial size for usage as a seed feature map.

\begin{equation}
\small
D_{KL} \; (\, N(\mu(\varphi_{t}), \; \Sigma(\varphi_{t} \,)\; || \; N(\,0, I\,))
\label{eq:txt}
\end{equation}


==> 4_ProposedMethod.tex <==
\section{Methodology}
\label{method}

Multi-modal Conditional GAN (MC Gan)의 전반적인 모델 구조는 Fig \ref{fig:arch}.와 같다.
In here, a Generator and a Discriminator is based on \cite{mao2017least,zhang2017stackgan} configured Synthesis block. 
Sec \ref{sec:synthesis-block}. 에서는 우리가 새롭게 제안하는 synthesis block 의 특징과 Sec \ref{sec:arch}. 에서는 전체 모델 구조와 이를 위한 loss function 정의에 대해 소개한다.

\begin{figure}
\centering
\begin{tabular}{c}
\bmvaHangBox{
\includegraphics[width=0.9\linewidth]{Method_img/model_arch.pdf}
}
\end{tabular}
\caption{ Overall structure of the proposed method }
\label{fig:arch}
\end{figure}


\subsection{Synthesis Block}
\label{sec:synthesis-block}

\begin{figure}
  \centering
  \begin{adjustbox}{width=\textwidth}
    \begin{tabular}{c p{0.3\textwidth}}
     \multicolumn{1}{c}{\multirow{5}[0]{*}{ 
    \bmvaHangBox{\includegraphics[width=0.7\textwidth]{Method_img/synthesis_block.pdf}}}} 
    &\bmvaHangBox{\includegraphics[width=0.3\textwidth]
{Method_img/Pacific_Loon_0038_75526_64_sentence2.png}}  \\
          & \tiny{The swan with a black crown and red eyes is swimming in the calm lake.}  \\
 &\multicolumn{1}{c}{(b)} \\
    &  \bmvaHangBox{\includegraphics[width=0.3\textwidth]
{Method_img/Golden_Winged_Warbler_0032_794849_64_sentence2.png}} \\
          & \tiny{This bird has yellow crown and gray feathers on the breast and long tail feather.}\\
           (a)   & \multicolumn{1}{c}{(c)} \\
    \end{tabular}%
  \end{adjustbox}  
  \caption{synthesis block 구조 및 결과 이미지}
  \label{fig:synthesis-block}
  
\end{figure}%


Classification 문제에서 네트워크 디자인은 weighted layer 통해 생성된 출력 $H(x)$를 만들고 이를 최적화 시키는 방향으로 학습이 진행된다. 그러나 Residual block은 원래의 $x$ 를 skip-connection 이어주었기 때문에 출력과 입력의 차가 적어지는 기본적인 학습 방향을 제시한다. 그러므로 최적화 하기가 어려운 깊은 레이어을 가져도 쉽게 좋은 solution을 찾아낸다.  ResNet 경우 처럼, 네트워크 디자인에서 기본적인 방향을 제시하는 것은 올바른 학습을 위해 중요하다. Base-image 를 기반으로 새로운 이미지를 만드는 문제에서는 새로운 object 를 생성할 때 기존의 Base-image를 무시하거나 전경과 배경이 겹치지 않도록 학습방향을 제시해야 한다. 


이를 위해 Fig \ref{fig:synthesis-block}. (a)처럼 Residual block 의 skip-connection 대상이 되는 identity matrix 를 각 resolution에 맞는 배경의 feature map 으로 변경하여 지속적으로 배경 정보를 제공하도록 하고 이를 BG라 한다. Residual block 에 해당되는 input $x$ 는 이전 layer 에서 나온 feature map 으로 두고 이를 FG라 한다. 단 첫번째 synthesis-block 의 input x 는 \cite{zhang2017stackgan, Han17stackgan2} 에서 이용한 방법을 따라 object 생성을 위해 넣어준 noise와 text의 embedding feature를 연결한 뒤 fully connected layer을 통과시켜 만든 feature map 으로 한다. BG와 FG의 feature map 의 크기는 동일하며 weighted layer 를 통과한 $FG$ 의 feature map dimension 을 2배로 만든다. 그래서 절반은 switch로 쓰고 절반은 이미지를 생성하기 위한 feature map으로 쓴다. 이를 통해 switch 부분은 object가 생성되는 영역을 알려준다. switch feature map은 sigmoid 함수를 통과 한 후 배경의 feature map과 elementwise multiplication 을 수행하여 생성될 이미지에서 배경을 가져올 영역의 정보만 남긴다. 최종적으로 억제된 배경과와 weighted layer 를 통과한 이전 layer의 feature map을 서로 elementwise addition 을 한 후 upsampling 을 수행한다.

Synthesis Block 은 generator 에서 만들어진 이미지의 배경과 base image의 배경을 비교하는 loss가 있기 때문에, object가 생기는 영역에 배경정보를 억제시키는 네트워크의 학습방향을 제공한다. 이를 통해 생성된 이미지가 base image를 반영하게 되고, 새로 생긴 영역과 원래의 영역이 겹쳐지지 않도록 학습이 가능해진다.  Fig \ref{fig:synthesis-block}. (b), (c) 는 위치를 지정한 배경 이미지, generator 를 통해 생성한 이미지, generator를 통해 생성된 마스크 그리고 sigmoid 를 통과한 후 switch map을 시각화 한 것이다. Switch 는 BG가 새로 생긴 object와 변경된 배경영역은 attention 을 덜 하도록 만든다. 이를 통해 model은 원래의 배경을 그대로 두고 알맞은 자리에 적절한 pose 를 가지고 object를 생성 하지만 필요한 경우 배경을 적절히 변경하여 자연스러운 합성을 가능하게 한다. Fig \ref{fig:synthesis-block} (b). 는 object 와 배경이 자연스럽기 때문에 원래의 배경을 변화시키지 않기 때문에 object 가 아닌 배경영역은 attention 이 많이 된 것을 switch map 에서 확인 할 수 있다. 반면에 Fig \ref{fig:synthesis-block} (c). 는 공중에 새가 있는 것은 부자연스럽기 때문에 generator 가 나뭇가지를 생성해준다. 이때 새로 생긴 나뭇가지와 원래 배경이 겹치면 안되기 때문에 switch map에서 알 수 있듯이 나뭇가지영역에는 배경 정보를 억제한다.
\hj{ 교수님: sigmoid 에 들어가는 input 에 W 곱하여 그 효과를 보기, 각 block 단계마다 이미지가 어떻게 생성되가는지 Arch 에 example로 보여주기}




\subsection{Network Design and Loss Definition}
\label{sec:arch}

MC Gan 은 base image 의 image feature 와 text 의 text embedding feature 를 synthesis block 을 통해 합성한다. 여기서 text embedding 후 처음 seed feature map 을 만드는 방법은 Sec \ref{sec:Background}. 에서 언급했듯이 \cite{zhang2017stackgan,Han17stackgan2} 에서 제안한 방법을 따르고, Base image 로 부터 합성하고 싶은 영역을 crop 하여 MC Gan 의 input image 로 넣어준다.
Input image spatial 크기가 $W \times H$ 이고 Synthesis Block 의 개수를 $N$개 라 한다. 
fully connected layer 를 통과한 seed feature map 크기는 $1024 \times\frac{W}{2^N} \times \frac{H}{2^N}$ 가 되며 Up Block 하나씩 통과할 때 마다 resolution 은 2배씩 커진다. 
Up Block 은 Nearest 방법으로 resolution을 2배 올린 뒤 $3\times3$ kernel 크기의 convolution과 Batch Normalization + Relu 을 통해 smoothing 하고 매 step 마다 channel 를 절반으로 줄인다.
반대로 Image feature 만드는 방법은 non-linear function 을 이용하지 않았으며, 각 단계는 $stride = 2$ and $3\times3$ kernel 을 가진 Convolution filter 와 Batch Normalization 으로만 이루어져 있다. 각 단계를 통과 할 때 마다 spatial resolution 은 절반이 되고 channel 수는 2배가 되어 각 단계에 맞는 Synthesis Block 에 들어간다. 최종적인 feature map 은 $64*W*H$ 가 되어 RGB image 와 segmentation mask 를 가진 4 channel 로 전환된다.

Discriminator 는 image-mask-text pair를 input 로 가진다. image 와 mask 는 convolution + Batch normalization + Leaky Relu 로 이루어진 Down Block 을 통해 $4\times4$ resolution 으로 down sampling 되어 image code 와 image-mask code를 따로 만든다. image-mask code 는 conditional Augmentation technique 으로 만든 conditioning Gaussian distribution 에서 추출한 sample $\hat{c_0}$ 를 image-mask code 의 spatial size 만큼 replicate 한 후 concate 한다. concate 한 image-mask-text code 는 $3\times3$ convolution + Batch Normalization + LeakRelu 로 이루어진 Joint convolution block 으로 들어가 종합적인 encoding 을 만든다. 3가지 image code, image-mask code, image-mask-text code \cite{mao2017least} 에서 제안한 Discriminator로 학습한다. 이때 Discriminator는 Tab \ref{tab:netD_pair}. 따라 4가지 pair 로 학습하여 fake image, fake mask and mismatching text 를 구분한다.

\begin{table}[h]
  \centering
  
    \begin{tabular}{l|l|l}
    1)    & img1, mask1, text1 & real image with matching mask and text \\
    2)    & img2, mask1, text1 & real image with matching mask but mismatching text \\
    3)    & img1, mask2, text1 & real image with mismatching mask but mismatching text  \\
    4)    & fake img, fake mask, text1 & fake image with fake mask and matching text \\
    \end{tabular}%
    \caption{Discriminator D with 4 types of input pairs}
  \label{tab:netD_pair}%  
\end{table}%

Generator를 학습할 때는 위에서 언급한 Discriminator 뿐만 아니라 text encoding 과 background reconstruction 을 위한 regularization term 이 추가 된다. Text encoding 을 위한 term 은 Sec \ref{sec:Background}. 에서 언급한 KL divergence loss 를 이용한다. Background reconstruction loss 는 배경이미지를 합성하기 위해 base image 의 feature 를 추출하는데 영향을 주며 switch 에서 어떤 부분을 가져와야 하는지 방향을 제시한다. generated 된 Mask 를 이용하여 fake image 와 base image 에서 object 부분을 제외한 영역을 가져와 L1 loss 로 학습한다. 최종적인 loss function 은 Eq \ref{eq:loss}. 과 같다.
\begin{equation}
\small
\begin{aligned}
L_D \; = \;\mathds{E}_{x_1,s_1,t_1\sim p_{data}}\;[\, ({D((x_1,s_1,\varphi(t_1)))-1})^2 \,] 
\; + \; \mathds{E}_{x_2,s_1,t_1\sim p_{data}}\;
[\, {D(x_2,s_1,\varphi(t_1))}^2 \,]\\
\; + \;\mathds{E}_{x_1,s_2,t_1\sim p_{data}}\;
[\, {D(x_1,s_2,\varphi(t_1))}^2 \,]
\; + \;\mathds{E}_{\hat{x},\hat{s}\sim p_{G(I,\hat{c_0},z)}}\;
[\, {D(G(I,\hat{c_0},z))}^2 \,]\\
L_G \; = \;\mathds{E}_{\hat{x},\hat{s}\sim p_{G(I,\hat{c_0},z)}}\;
[\, ({D(G(I,\hat{c_0},z)-1)})^2 \,] \; + \; 
\lambda_{1} \, D_{KL} \; (\, N(\mu(\varphi_{t_{1}}), \; \Sigma(\varphi_{t_{1}} \,)\; || \; N(\,0, I\,)) \\ \; + \; 
\lambda_2 \, [|(\hat{x} \odot \hat{s}) - (\hat{I} \odot \hat{s})]]
\qquad \qquad \qquad \bm{* (\hat{x},\hat{s}) \; = \; G(I,\hat{c_0},z)}
\label{eq:loss}
\end{aligned}
\end{equation}































==> 4_ProposedMethod_EN_old.tex <==
\section{Methodology}
\label{method}



\begin{figure}[t]
\centering
\begin{tabular}{c}
\bmvaHangBox{
\includegraphics[width=0.9\linewidth]{Method_img/model_arch.pdf}
}
\end{tabular}
\caption{ Overall structure of the proposed method }
\label{fig:arch}
\end{figure}

Fig. \ref{fig:arch} represents the \nj{overall structure of the proposed MC-GAN.}
\hj{MC-Gan encodes input text sentence to text embedding $\varphi(t)$ using \citet{reed2016txt_emb}'s method.
And we follow the proposed method in \cite{zhang2017stackgan,Han17stackgan2} to make seed feature map.
After then, we use synthesis block to prevent overlap between generated object and background from the seed feature map and image feature step by step and we finally generate natural image $\hat{x}$ and mask $\hat{s}$. 
In Sec~\ref{sec:synthesis-block} we describe the characteristics of the proposed synthesis block. In \ref{sec:arch}.
we introduce the \yj{detailed} model structure and \yj{a training strategy of the network}.   
 }
% \nj{Fig 2에 대한 좀 더 자세한 설명이 필요함. 각각의 block이 대략적으로 어떤 역할을 하며 그림에서의 $\varphi(t), x, \hat{x}$ 등이 무엇을 의미하는지 자세히 설명할 것. 이러한 모델을 왜 선정하게 되었는지에 대한 당위성에 대한 대략적인 설명이 필요. }


% \yj{Brief explanation of the process?}
% Here, a Generator and a Discriminator is based on \cite{mao2017least,zhang2017stackgan}, and a newly proposed Synthesis block \yj{is added to the model why?}. In Sec~\ref{sec:synthesis-block} we describe the characteristics of the proposed Synthesis block. In \ref{sec:arch}. we introduce the \yj{detailed} model structure and 
% %\loss function definition 
% \yj{a training strategy of the network}. % for training the network.  

\subsection{Synthesis Block}
\label{sec:synthesis-block}

\begin{figure}[t]
  \centering
  \begin{adjustbox}{width=\textwidth}
    \begin{tabular}{c m{0.3\textwidth}}
     \multicolumn{1}{c}{\multirow{5}[0]{*}{ 
    \bmvaHangBox{\includegraphics[width=0.7\textwidth]{Method_img/synthesis_block.pdf}}}} 
    &\bmvaHangBox{\includegraphics[width=0.3\textwidth]
{Method_img/Pacific_Loon_0038_75526_64_sentence2.png}}  \\
          & \tiny{The swan with a black crown and red eyes is swimming in the calm lake.}  \\
 &\multicolumn{1}{c}{(b)} \\
    &  \bmvaHangBox{\includegraphics[width=0.3\textwidth]
{Method_img/Golden_Winged_Warbler_0032_794849_64_sentence2.png}} \\
          & \tiny{This bird has yellow crown and gray feathers on the breast and long tail feather.}\\
           (a)   & \multicolumn{1}{c}{(c)} \\
    \end{tabular}%
  \end{adjustbox}  
  \caption{synthesis block and result image}
  \label{fig:synthesis-block}
  
\end{figure}%


%In %the
%\yj{usual} classification problem, \yj{the network $H(x)$ is designed to have }a weighted \yj{deep?} layer and the learning direction\yj{?} %proceeds 
%to optimize $H(x)$. 
%Since the residual block has connection between the original input $x$ and the output $H(x)$, 
%the basic learning direction is set difference between the output and the input to become smaller.
%\yj{the residual block induces the difference between the output and the input smaller. right?}
%Therefore, the network easily finds a good solution even if it has a difficult deep layer to optimize. 
%As in the case of ResNet, it is important for optimization to suggest basic learning directions in network design.
%When the model create a new object, it must have a default learning direction that does not ignore the existing base image or overlap between the object and the background in synthesizing problem based on input image.
%\yj{I dont know what this section saying - one concrete explanation for using the resblock How it attached to the model and why - I think we can ommit this part.}

\yj{Figure \ref{fig:synthesis-block} (a) \nj{describes} the framework of the proposed \nj{synthesis} block. 
As \nj{can be seen} in the figure, the synthesis block is defined similar to the Residual skip-connection network \citet{he2016resnet}.
In the synthesis block, \nj{the background (BG)} feature controlled by a sigmoid switch is attached to the \nj{foreground (FG)} feature map which passes $H(x)$: (FG is x and H(x) will be conv-bn-leaky Relu - conv- BN block)}. \nj{??}
\yj{
%We call the background information \yj{as} BG. 
The input $x$ of the Residual block is replaced with the feature map from the previous layer and this is called the FG.} 
%To do this, we change the identity matrix, which is a target of the skip-connection in a Residual block, to a background feature map corresponding to each resolution 
%for 
%\yj{to} continuously \yj{preserve}%provision of 
%the background information.
\yj{This block is proposed in our problem to well preserve the information of the background part of \nj{an} image.}

The first input $x$ of the \nj{synthesis} block \yj{is derived from} the method\yj{which method?} used in \cite{zhang2017stackgan, Han17stackgan2}. 
\yj{In which part?->we should mention it. }
After combining the random noise and conditioning augmented text embedding feature, the combined feature map passes through a fully connected layer to create a new seed feature \nj{which is used by the model. ?? 문장이 어색함. }
The \nj{sizes} of the \nj{BG and FG} feature \nj{maps are} the same, and the \nj{depth of FG feature map is doubled as it pass through the convolution layers.} %passed through the weighted layer is doubled. 
\nj{A} half of \nj{the} doubled feature \nj{map denoted as switch in the figure is used as an input to the} switch, \nj{while} the other half is \nj{forwarded to} generate an image. 
The switch \nj{determines what amount of BG information should be retained for the next synthesis block.} 
%region where the object is created and where the region is retained. 
After switch feature \nj{map is} activated by \nj{the} sigmoid function, \nj{it} is element-wise multiplied with \nj{the} background feature map for \nj{the} suppression of background information where the object is to be generated. 
Finally, \nj{the spatial dimension of feature map is doubled by the upsampling block} after element-wise addition of the suppressed background \nj{feature map} and the foreground feature map. 


Because the \nj{synthesis block has an} \yj{$\ell1$ loss} comparing the background of created fake image with the background of the base image, the switch provides a basic network learning direction\yj{learning direction->any other proper word?} that suppresses the background information of the area where the object is generated. 
Therefore, a visualized switch map has the opposite \yj{concept to that of }
%image of 
the segmentation mask.% in general. 
This allows the generated image to reflect the base image and enable network to learn that the new object does not overlap with the original background. 
Fig \ref{fig:synthesis-block} (b), (c) is visualization of a cropped background image from specific location. \yj{captions should be added into the Fig2.}
%,a result image and mask by the generator and a switch map activated by sigmoid function. 
The switch makes BG less attention to the region of object and adjusted background. 
This allows the model to generate an object with the appropriate pose at the right spot \yj{with} appropriately \yj{compositing the original background image}.% but if necessary, changes the background appropriately for natural compositing.
Fig \ref{fig:synthesis-block} (b) does not change the original background because the object and background are natural.
So the picture shows that the background region are highly activated from switch except region of the object.
On the other hand, a picture of bird standing on the air \yj{in Fig \ref{fig:synthesis-block} (c)} is unnatural.
So, the generator adds a branch in the figure. 
At this time, since the original background should not overlap with the new background, the background information of the new branch area is suppressed as shown in the switch map.

\hj{ 교수님:각 block 단계마다 이미지가 어떻게 생성되가는지 Arch 에 example로 보여주기}
\hj{encoder decoder}


\subsection{Network Design and Loss Definition}
\label{sec:arch}

The MC Gan synthesizes the image feature of the base image and the text embedding feature of the text through a Synthesis block. 
\hj{MC-Gan encodes input text sentence using \citet{reed2016txt_emb}'s method. However, the vector $\varphi(t)$ \yj{generated} by the text embedding method \yj{lies on} high dimension \yj{manifold} and the number of data is small, \cite{zhang2017stackgan,Han17stackgan2} points out this problem and proposes Conditioning Augmentation method and fully connected layer to make initial seed feature map.}
Here, the method of creating the first seed feature map after text embedding follows the method proposed in \cite{zhang2017stackgan,Han17stackgan2} mentioned in Sec \ref{sec:Background}, and the cropped region from the base image is the input image of MC Gan. 
The spatial size \yj{of the input image} is $ W \times H $ and the number of synthesis blocks is $ N $. The size of the seed feature map after fully connected layer is $1024 \times\frac{W}{2^N} \times \frac{H}{2^N}$ and the resolution is doubled with each pass through a decoder. 
The decoders for upsampling use\yj{s} the nearest neighborhood method to double the resolution, \yj{with using} the convolution of $ kernel \; size = 3\times3 $.
Batch Normalization \yj{followed by} Relu is added to improve the quality of image and \yj{also} halve the channel of feature map \yj{in} every step. 
Conversely, the method of creating an image feature does not use any non-linear function, and each step consists of a convolution layer with with $ stride = 2 $ and $ kernel \; size = 3\times3 $  and batch normalization . 
At each step, the spatial resolution is halved and the number of channels is doubled to 
%enter the 
\yj{match the feature dimensions?} in Synthesis block. The final feature map is $ 64\times W \times H $ and is converted into 4 channels with RGB image and segmentation mask.


The Discriminator has an image-mask-text pair as an input. The generated image and mask are downsampled to $ 4\times4 $ resolution through the Down block consisting of $ convolution + Batch \;normalization + Leaky \;Relu $ into image code and image-mask code separately. The image-mask code associates with the replicated sample $ \ hat {c_0} $ , which is extracted from the conditioning Gaussian distribution devised by the conditional augmentation technique~\yj{[]}, as much as the spatial-size of the image-mask code. \hj{????? image-mask code 는 conditional Augmentation technique 으로 만든 conditioning Gaussian distribution 에서 추출한 sample $\hat{c_0}$ 를 image-mask code 의 spatial size 만큼 replicate 한 후 연결한다.} We apply a convolution layer to the associated image-mask-text code, then perform Batch normalization and Leaky Relu activation for making a comprehensive encoding. The image code, image-mask code, and image-mask-text code are learned by method proposed in \citet{mao2017least}. At this time, Discriminator learns 4 pairs according to Tab \ref{tab:netD_pair}. and distinguishes fake image, fake mask and mismatching text.

\begin{table}[h]
  \centering
  
    \begin{tabular}{l|l|l}
    1)    & img1, mask1, text1 & real image with matching mask and text \\
    2)    & img2, mask1, text1 & real image with matching mask but mismatching text \\
    3)    & img1, mask2, text1 & real image with mismatching mask but mismatching text  \\
    4)    & fake img, fake mask, text1 & fake image with fake mask and matching text \\
    \end{tabular}%
    \caption{Discriminator D with 4 types of input pairs}
  \label{tab:netD_pair}%  
\end{table}%

When learning the generator, a regularization term is added for conditioning Gaussian distribution and background reconstruction. The term for text encoding $\varphi(t)$ uses the KL divergence loss mentioned in Sec \ref{sec:Background}. Background reconstruction loss affects the feature extraction of the base image to synthesize the background image and suggests the direction of the switch which part should be taken. Using the generated mask $\hat{s}$ and morphology operation, the area excluding the object part and boudary in the fake image $\hat{x}$ and the base image $I$ is taken and learned as L1 loss. The final loss function is equal to Eq \ref{eq:loss}.
\begin{equation}
\small
\begin{aligned}
L_D \; = \;\mathds{E}_{x_1,s_1,t_1\sim p_{data}}\;[\, ({D((x_1,s_1,\varphi(t_1)))-1})^2 \,] 
\; + \; \mathds{E}_{x_2,s_1,t_1\sim p_{data}}\;
[\, {D(x_2,s_1,\varphi(t_1))}^2 \,]\\
\; + \;\mathds{E}_{x_1,s_2,t_1\sim p_{data}}\;
[\, {D(x_1,s_2,\varphi(t_1))}^2 \,]
\; + \;\mathds{E}_{\hat{x},\hat{s}\sim p_{G(I,\hat{c_0},z)}}\;
[\, {D(G(I,\hat{c_0},z))}^2 \,]\\
L_G \; = \;\mathds{E}_{\hat{x},\hat{s}\sim p_{G(I,\hat{c_0},z)}}\;
[\, ({D(G(I,\hat{c_0},z)-1)})^2 \,] \; + \; 
\lambda_{1} \, D_{KL} \; (\, N(\mu(\varphi_{t_{1}}), \; \Sigma(\varphi_{t_{1}} \,)\; || \; N(\,0, I\,)) \\ \; + \; 
\lambda_2 \, [|(\hat{x} \odot ( f \circ\hat{s})) - 
(\hat{I} \odot (f \circ \hat{s}))]]
\qquad \qquad \qquad \bm{* (\hat{x},\hat{s}) \; = \; G(I,\hat{c_0},z)}
\label{eq:loss}
\end{aligned}
\end{equation}

\yj{Here, 설명 of the terms in the equation 3. 각 기호들은 무었인가요?}































==> 5_Experiment.tex <==
\section{Experiment}
\label{Exp}
뭐야 머 있고 간략히 실험 내용 써두기

\subsection{Dataset and training details}
\label{data}
우리는 text to image generation work 에 널리 쓰이는 Caltech-200 bird dataset \cite{WahCUB_200_2011} 와 Oxford-102 flower dataset \cite{Nilsback08}를 이용하여 비슷한 문제를 정의한 Dong \etal \cite{dong2017semantic} 을 baseline method 로 비교 실험을 한다. 

Caltech-200 bird dataset 은 200 종류의 새 사진 있으며, train 으로 150종류 test로 50종류로 나누어져 있고 총 11788 장의 이미지와 segmentaiton mask를 제공한다.
Text 은 Reed \etal \cite{reed2016txt_emb}이 각 이미지당 10개의 caption 을 모은 추가 dataset을 이용한다. 각 caption 들은 새의 모습, 색깔 등을 설명한다.
Oxford-102 flower dataset 은 102 종류의 꽃 사진이 있으며, train으로 82종류 test로는 20 종류로 나누어져 있으며 총 8189장 이미지를 제공한다. 그러나 \cite{Nilsback08} 은 사람이 만든 정확한 segmentation mask 가 없기 때문에 Nilsback \etal \cite{Nilsback07Seg} 이 연구한 segmentation method 결과를 ground truth 로 쓴다.
이것은 사람이 직접 만든 dataset 이 아니기 때문에 일부분 부정확한 mask가 있는 문제가 있다. 
또한 사진의 대부분이 전경이 차지하기 때문에 배경사진으로는 웹에서 keyword 'flower leaf' or 'flower foliage' 를 통해 나온 이미지를 추가 dataset 으로 이용하였으며, train 으로 1217장 test 로 135장 이용하였다.
Text 또한 Reed \etal \cite{reed2016txt_emb}이 각 이미지당 10개씩 caption을 만든 것을 이용하며, 이 또한 꽃의 모양 및 색깔에 대해 설명한다.

\subsection{Comparison with the Baseline Method}
\label{compare}
 
공정성을 위해 우리는 200번 마다 learning rate 를 감소시켰고 우리가 학습한 epoch만큼 모델을 학습하였다 (dong et al의 work을?).
Fig \ref{fig:bird} and Fig \ref{fig:flower}는 input base image 와 text 에 따른 결과를 보여준다. 
\citet{dong2017semantic}은 flower dataset 에서 text 조건에 따른 이미지 생성을 보여주지만, base image를 완전히 무시하고 이미지를 생성한다는 것을 볼 수 있으며, 더 어려운 bird dataset은 대부분 경우 이미지가 제대로 생성이 안되거나, 배경을 무시하고 생성이 되거나, 배경만 reconstruction 하는 것을 알 수 있다. 
\begin{figure}[t]
  \centering
%     \begin{tabular}{m{0.125\textwidth}m{0.125\textwidth}m{0.125\textwidth}m{0.125\textwidth}|m{0.125\textwidth}m{0.125\textwidth}m{0.125\textwidth}m{0.125\textwidth}}
\begin{tabular}{cccccccc}
%  \multicolumn{1}{c}{ \centering{base image}}
%     & \multicolumn{2}{c}{\centering{our result} }
%     &\multicolumn{1}{c}{\centering{baseline method\cite{dong2017semantic}}} 
   
%    &\multicolumn{1}{c}{ \centering{base image}}
%     & \multicolumn{2}{c}{\centering{our result} }
%     &\multicolumn{1}{c}{\centering{baseline method\cite{dong2017semantic}}} \\
    
    \multicolumn{1}{m{0.125\textwidth}}{ \centering{Base}}
    & \multicolumn{2}{m{0.15\textwidth}}{\centering{Our result} }
    &\multicolumn{1}{m{0.125\textwidth}}{\centering{Method\cite{dong2017semantic}}} 
 \vline  
   &\multicolumn{1}{m{0.125\textwidth}}{ \centering{Base}}
    & \multicolumn{2}{m{0.15\textwidth}}{\centering{Our result} }
    &\multicolumn{1}{m{0.125\textwidth}}{\centering{Method\cite{dong2017semantic}}} \\
    
    
    \multicolumn{4}{c}
    {\bmvaHangBox{\includegraphics[width=0.45\textwidth]{MC_bird/Acadian_Flycatcher_0009_29155_s8.png}}}  \vline  
    & \multicolumn{4}{c}
    {\bmvaHangBox{\includegraphics[width=0.45\textwidth]{MC_bird/Black_Billed_Cuckoo_0024_795331_s8.png}}} \\
    \multicolumn{4}{m{0.45\textwidth}}{\centering\tiny{This bird has wings that are brown and has a yellow belly.}}  \vline   
& \multicolumn{4}{m{0.45\textwidth}}{\centering\tiny{This bird has wings that are black and has a white belly.}} \\


    \multicolumn{4}{c}
     {\bmvaHangBox{\includegraphics[width=0.45\textwidth]{MC_bird/Black_Footed_Albatross_0033_796086_s8.png}}}  \vline  
     & \multicolumn{4}{c}
     {\bmvaHangBox{\includegraphics[width=0.45\textwidth]{MC_bird/Purple_Finch_0005_27512_s6.png}}}\\
    \multicolumn{4}{m{0.45\textwidth}}{\centering\tiny{This bird has a brown crown as well as a long brown bill.}} \vline  
    & \multicolumn{4}{m{0.45\textwidth}}{\centering\tiny{This is a red bird with a gray cheek patch and gray wings and tail.}} \\
    
    
    \multicolumn{4}{c}
     {\bmvaHangBox{\includegraphics[width=0.45\textwidth]{MC_bird/Tree_Sparrow_0011_122964_s3.png}}}  \vline  
     &\multicolumn{4}{c}
     {\bmvaHangBox{\includegraphics[width=0.45\textwidth]{MC_bird/White_Breasted_Kingfisher_0054_73587_s3.png}}}\\
    \multicolumn{4}{m{0.45\textwidth}}{\centering\tiny{This bird has a white belly, grown wing and grey head.}}   \vline     
    & \multicolumn{4}{m{0.45\textwidth}}{\centering\tiny{This bird has a bright blue outline on its coverts and retrices.}} \\
    \end{tabular}%
    \caption{Image synthesis samples generated from our MC Gan ($128\times 128$) and baseline method \cite{dong2017semantic} ($64\times 64$) using Caltech-cub200}  
  \label{fig:bird}%
\end{figure}%


\begin{figure}[t]
  \centering
\begin{tabular}{cccccccc}
    
    \multicolumn{1}{m{0.125\textwidth}}{ \centering{Base}}
    & \multicolumn{2}{m{0.15\textwidth}}{\centering{Our result} }
    &\multicolumn{1}{m{0.125\textwidth}}{\centering{Method\cite{dong2017semantic}}} 
 \vline  
   &\multicolumn{1}{m{0.125\textwidth}}{\centering{Base}}
    & \multicolumn{2}{m{0.15\textwidth}}{\centering{Our result} }
    &\multicolumn{1}{m{0.125\textwidth}}{\centering{Method\cite{dong2017semantic}}} \\
    
    
    \multicolumn{4}{c}
    {\bmvaHangBox{\includegraphics[width=0.45\textwidth]{MC_flower/03096_s0.png}}}  \vline  
    & \multicolumn{4}{c}
    {\bmvaHangBox{\includegraphics[width=0.45\textwidth]{MC_flower/03101_s2.png}}} \\
    \multicolumn{4}{m{0.45\textwidth}}{\centering\tiny{This flower has petals that are pink with patches of yellow
a pink velvety flower with white stamen and curled petals.}}  \vline   
& \multicolumn{4}{m{0.45\textwidth}}{\centering\tiny{The flower has red and yellow petals that are small and round.}} \\


    \multicolumn{4}{c}
     {\bmvaHangBox{\includegraphics[width=0.45\textwidth]{MC_flower/03106_s7.png}}}  \vline  
     & \multicolumn{4}{c}
     {\bmvaHangBox{\includegraphics[width=0.45\textwidth]{MC_flower/03117_s0.png}}}\\
    \multicolumn{4}{m{0.45\textwidth}}{\centering\centering\tiny{This flower has white petals as well as a green pedicel.}} \vline  
    & \multicolumn{4}{m{0.45\textwidth}}{\centering\tiny{Column of pale pink flowers stacked atop each other with curled petals.}} \\
    
    
    \multicolumn{4}{c}
     {\bmvaHangBox{\includegraphics[width=0.45\textwidth]{MC_flower/03118_s1.png}}}  \vline  
     &\multicolumn{4}{c}
     {\bmvaHangBox{\includegraphics[width=0.45\textwidth]{MC_flower/06625_s5.png}}}\\
    \multicolumn{4}{m{0.45\textwidth}}{\centering\tiny{This are bright yellow flowers with tongues are in a cluster and that cluster often forms spikes.}}   \vline     
    & \multicolumn{4}{m{0.45\textwidth}}{\centering\tiny{These are pretty bell-shaped purple flowers with yellow anthers and white stigma.}
} \\
    \end{tabular}%
    \caption{Image synthesis samples generated from our MC Gan ($128\times 128$) and baseline method \cite{dong2017semantic} ($64\times 64$) using Oxford-flower102}  
  \label{fig:flower}%
\end{figure}%



\subsection{Comparison with other Synthesis Problem}
\label{other-synthesis}
우리는 Synthesis block이 배경 이미지에 object 여부에 상관없이 안정적으로 이미지를 합성하는 것을 \citet{dong2017semantic}이 제시한 문제를 해결함으로서 보여준다.  \citet{dong2017semantic} 은 object가 포함된 base image 와 target text를 넣어주면 text와 관련있는 부분은 내용에 맞게 바꾸어주고 관련이 없는 부분은 유지하는 것을 목표로 한다.  학습은 \citet{dong2017semantic}와 동일하게 segmentation mask를 이용하지 않고 같은 text embeding을 이용하였으며, 100epoch 마다 0.5씩 learning rate 를 감소하고 600 epoch 까지 하였다. 그러나 generator와 discriminator network는 우리가 제안한 구조를 이용하였으나 discriminator pair loss 는 \citet{dong2017semantic}과 동일하게 image-text pair 만 고려하였다.

\citet{dong2017semantic}은 배경이미지가 복잡하지 않은경우 잘 되지만 배경이 복잡한 경우 이미지가 collapsed 되고 text과 관련없는 부분인 배경도 많이 변경된다. 그러나 우리가 제안한 Synthesis block 을 이용한 generator 는 배경이 복잡한 상황에서도, 안정적으로 object, background 모두 형태를 유지하며 text와 관련 없는 배경부분이 변경되는 경우가 거의 없다. segmentation mask 를 이용하지 않아도 각 resolution 마다 image 정보를 주어 배경을 guide 하기 때문에 target text 와 관련이 없는 배경부분이 유지되고 object의 색이 잘 변하지 않아도 적어도 형태가 이상하게 변형되지 않았다. 

\begin{figure}
  \centering
      \begin{tabular}{p{4cm} | c | c}
   
          & \multicolumn{1}{c|}{Baseline method\cite{dong2017semantic}} & \multicolumn{1}{c}{Our result} \\
         
    \small{Original} 
    &  \bmvaHangBox{\includegraphics[width=4cm]{iccv_transfer_mine/original.jpg}}     
&  \bmvaHangBox{\includegraphics[width=4cm]{iccv_transfer_mine/original.jpg}}\\ 
    \scriptsize{This small bird has a blue crown and white belly.} 
    &\bmvaHangBox{\includegraphics[width=4cm]{iccv_transfer_dong/output_0.jpg}}
&\bmvaHangBox{\includegraphics[width=4cm]{iccv_transfer_mine/output_0.jpg}}  \\ 
   \scriptsize{This small yellow bird has grey wings, and a black bill. } 
    &\bmvaHangBox{\includegraphics[width=4cm]{iccv_transfer_dong/output_1.jpg}}
&\bmvaHangBox{\includegraphics[width=4cm]{iccv_transfer_mine/output_1.jpg}}  \\ 
   \scriptsize{A small brown bird with a brown crown has a white belly. } 
    &\bmvaHangBox{\includegraphics[width=4cm]{iccv_transfer_dong/output_2.jpg}}
&\bmvaHangBox{\includegraphics[width=4cm]{iccv_transfer_mine/output_2.jpg}}  \\
   \scriptsize{This black bird has no other colors with a short bill. }
    &  \bmvaHangBox{\includegraphics[width=4cm]{iccv_transfer_dong/output_3.jpg}}     
    & \bmvaHangBox{\includegraphics[width=4cm]{iccv_transfer_mine/output_3.jpg}} \\ 
    \scriptsize{An orange bird with green wings and blue head.}
    &  \bmvaHangBox{\includegraphics[width=4cm]{iccv_transfer_dong/output_4.jpg}}    
    &  \bmvaHangBox{\includegraphics[width=4cm]{iccv_transfer_mine/output_4.jpg}}\\ 
  \scriptsize{A black bird with a red head.}
    &  \bmvaHangBox{\includegraphics[width=4cm]{iccv_transfer_dong/output_5.jpg}}  
    & \bmvaHangBox{\includegraphics[width=4cm]{iccv_transfer_mine/output_5.jpg}} \\ 
   \scriptsize{ This particular bird with a red head and breast and features grey wings.} 
    &  \bmvaHangBox{\includegraphics[width=4cm]{iccv_transfer_dong/output_6.jpg}}      
    & \bmvaHangBox{\includegraphics[width=4cm]{iccv_transfer_mine/output_6.jpg}} \\ 
    \end{tabular}%
    \caption{Zero-shot results of the baseline method \cite{dong2017semantic} and our method about Caltech-200 bird test dataset}
  \label{fig:zeroshot}%
\end{figure}%

\subsection{Interpolation and Variety Experiment}
\label{etc_exp}
text to image Gan에서는 text 정보를 가진 latent manifold 가 continuous 하게 학습되어야 다양한 문장에 알맞게 이미지 생성이 가능하다. 이를 위해 우리는 두개의 서로 다른 text embedidng 을 linear interpolation 통해 새로운 text embedding 으로 만들어 자연스럽게 변화하는지 실험을 하였다. Fig. \ref{fig:interpolation}. 은 같은 모델 같은 noise 조건 에서 자연스럽게 이미지가 합성된 결과를 보여준다. 
\begin{figure}
  \centering  
 {\bmvaHangBox{\includegraphics[width=0.95\textwidth]{Etc_exp/txt_interpolation.pdf}}}       
    \caption{Experiment of generated images of interpolation between text descriptions from same base image.}
  \label{fig:interpolation}%
\end{figure}%
GAN 에서는 이미지가 다양하고 안정적으로 생성되는 것이 매우 중요하다. 우리는 0 만 가진 noise 로 부터 1만 가지는 noise 로 점차적으로 변화시키면서 같은 text 와 image 조건에서 안정적이면서도 다양한 sample을 생성하는 실험하였다. text와 image 조건에 따라 약간의 차이가 있지만 보통 절반정도 성공적인 이미지가 합성되었으며, noise 에 따라 다양한 object와 조금씩 변형된 배경화면을 가진 결과물을 Fig \ref{fig:v_s} 는 보여준다.
% 다양한 이미지
\begin{figure}
  \centering  
    {\bmvaHangBox{\includegraphics[width=0.95\textwidth]{Etc_exp/variety_stability.pdf}}}   
     \caption{Variety and stability experiment from 0 to 1 noise}
  \label{fig:v_s}%
\end{figure}%



\subsection{Switch Experiment}
\label{swtich}
Synthesis block 의 switch 는 배경과 전경이 서로 overlap 되지 않도록 막아주는 역할을 한다. 이를 확인하기 위해 우리는 같은 base image, text embedding, noise로 부터 다르게한 activated switch from sigmoid  나온 이미지를 비교 하였다. 모든 switch 를 off 하여 배경정보가 더해지는 것을 막는 경우는 배경이 아에 사라지고 object와 변형된 배경만 있었다. 모든 switch 값을 0.5로 한 경우 배경이 reconstruction 되지만 object와 배경이 조금 overlap 된다. 마지막으로 모든 switch를 on 하여 원래의 배경 정보가 더해지는 경우 object 와 배경이 아에 overlap 되어 object가 제대로 보이지 않았다. 그러므로 switch는 현재의 image text 조건을 분석하여 flexible 하게 값을 조정하여 적절한 합성이 되도록 도움을 준다.
\begin{figure}
  \centering  
 {\bmvaHangBox{\includegraphics[width=0.95\textwidth]{Etc_exp/swtich0to1.pdf}}}       
    \caption{Experiment of generated images of switch transition in the Synthesis block}
  \label{fig:switch}%
\end{figure}%



\subsection{Inference}
\label{inference}
최종 합성 이미지
